Self-Paced Learning: an Implicit Regularization Perspective

Self-paced learning (SPL) mimics the cognitive mechanism of humans and animals that gradually learns from easy to hard samples. One key issue in SPL is to obtain better weighting strategy that is determined by minimizer function. Existing methods usually pursue this by artificially designing the explicit form of SPL regularizer. In this paper, we focus on the minimizer function, and study a group of new regularizer, named self-paced implicit regularizer that is deduced from robust loss function. Based on the convex conjugacy theory, the minimizer function for self-paced implicit regularizer can be directly learned from the latent loss function, while the analytic form of the regularizer can be even known. A general framework (named SPL-IR) for SPL is developed accordingly. We demonstrate that the learning procedure of SPL-IR is associated with latent robust loss functions, thus can provide some theoretical inspirations for its working mechanism. We further analyze the relation between SPL-IR and half-quadratic optimization. Finally, we implement SPL-IR to both supervised and unsupervised tasks, and experimental results corroborate our ideas and demonstrate the correctness and effectiveness of implicit regularizers.

==> paper/experiments/databases.tex <==
\begin{table} [tb]
	\footnotesize
	\caption{\small{Statistical Information of Databases.}}
	\centering
	\label{statistical_information_database}
	\begin{tabular}{|c|c|c|c|}
		\hline
		\textbf{Dataset} & \textbf{\#.Category} & \textbf{\#.Instance} & \textbf{\#.Feature} \\
		
		\hline
		Breast Wisconsion & 2 & 569 & 30 \\
		
		\hline
		Pima & 2 & 768 & 8 \\
		
		\hline
		Splice & 2 & 3175 & 60 \\
				
		\hline
		Spambase & 2 & 4601 & 57 \\
		
		\hline
		Phoneme & 2 & 5404 & 5 \\
		
		\hline
		Svmguide1 & 2 & 7089 & 4 \\
				
		\hline
	\end{tabular}
\end{table}

==> paper/experiments/table_classification_small_2.tex <==

\begin{table}[!tb]
	\footnotesize
	\centering
	\caption{
	\small{
	Classification accuracy (\%). The best results are highlighted in bold, respectively.}
	}
	\label{result_classification}
%	\setlength\tabcolsep{6.5pt}
	\renewcommand\arraystretch{1}
%	\begin{tabular}{c c c c c c c c c}
%	\begin{tabular}{|l| c| c| c|}
	\begin{tabular}{c| c c c}
		\hline
		\multicolumn{4}{c}{Without Label Noise} \\
		
		\hline
		Method & \tabincell{c}{Breast} & Spambase & Svmguide1 \\
		
		\hline
		
		\tabincell{l}{LR }			  & 97.36(2.22) &		92.35(1.47) &		95.39(0.95)  \\
		
		\hline
		\tabincell{l}{SPL-hard}    & 97.54(2.22) 	& 92.63(1.08) &		95.39(0.95) 	\\ 
%				
%		\hline
%		\tabincell{l}{SPL-linear}    & 98.25(1.65) 	& 92.83(1.44) 	& 95.51(1.04) 	\\ 
						
								
		\hline
		\tabincell{l}{SPL-mixture}    & 98.25(1.65) 	& 92.83(1.44) 	& 95.51(1.04) 	\\ 
				
		\hline
		\tabincell{l}{SPL-IR-huber}   & \textbf{98.77(1.19)} 	& 93.05(1.25) 	& 95.57(0.95) 	\\ 
				
		\hline
		\tabincell{l}{SPL-IR-L1-L2}   & 97.90(1.79) 	& 93.00(1.36) 	& 95.57(1.10) 	\\ 


		\hline
		\tabincell{l}{SPL-IR-cauchy}  & 98.42(1.54) 	& 93.09(1.41) 	& 95.65(1.01) 	\\ 
				
		\hline
		\tabincell{l}{SPL-IR-welsch}  & 98.25(1.65) 	& \textbf{93.13(1.34)} 	& \textbf{95.68(0.90)} 	\\ 

	
		%20
		\hline
		\multicolumn{4}{c}{With 20\% Random Label Noise} \\
		
		\hline
		Method & \tabincell{c}{Breast} & Spambase & Svmguide1 \\
		
		\hline
		
		\tabincell{l}{LR }			  & 92.08(2.96) &	89.28(1.66) &		91.52(0.65) \\
			
		\hline
		\tabincell{l}{SPL-hard}    & 96.13(2.15) 	& 89.81(1.61) 	& 92.72(1.12) 	\\ 
					
		\hline
		\tabincell{l}{SPL-mixture}    & 96.66(2.12) 	& 90.76(1.82) 	& 93.81(0.79) 	\\ 
				
		\hline
		\tabincell{l}{SPL-IR-huber}   & 96.84(2.33) 	& 90.92(1.65) 	& 93.54(0.75) 	\\ 
				
		\hline
		\tabincell{l}{SPL-IR-L1-L2}   & 94.72(2.89) 	& 90.09(1.65) 	& 92.83(0.71) 	\\ 


		\hline
		\tabincell{l}{SPL-IR-cauchy}  & 97.54(1.90) 	& 90.85(1.55) 	& 93.88(1.05) 	\\ 
				
		\hline
		\tabincell{l}{SPL-IR-welsch}  & \textbf{97.89(1.63)} 	& \textbf{91.37(1.37)} 	& \textbf{94.37(0.90)} 	\\ 
		
		\hline
		
	\end{tabular}
	%	\captionsetup{justification=centering}
\end{table}

==> paper/graph/graph_acc.tex <==
\begin{figure*}[tbh]
	\setlength{\abovecaptionskip}{0pt}
	\setlength{\belowcaptionskip}{-5pt}
	\centering
	\subfigure{\label{subfig:voc}
		\includegraphics[width=2.2in]{graph_results/voc/voc_mini_acc.jpg}
	}
	\subfigure{\label{subfig:movie}
		\includegraphics[width=2.2in]{graph_results/movies/movies_mini_acc.jpg}
	}
	%	\subfigure[Animal]{\label{subfig:movie}
	%		\includegraphics[width=2.2in]{graph_results/animal/animal_mini_acc.eps}
	%	}
	\subfigure{\label{subfig:bvcrbf1}
		\includegraphics[width=2.2in]{graph_results/3Sources/3sources_mini_acc.jpg}
	}
	\caption{Accuracy of the proposed model vs. \(\lambda\) and \(\beta\)}
	\label{fig:acc result}
\end{figure*}


==> paper/proposed_model/algorithm.tex <==

\begin{algorithm}
	\caption{: Algorithm for subproblem 2}
	\label{alg_for_p2}
	\begin{algorithmic}[1]
		\REQUIRE Multi-view data \(\bX^{v} \in R^{d_{v}\times n}\) and current sample weights $\bP^v \in R^{n \times n}$, (\(v = 1,\dots, m \)); parameters $\beta$ and $\rho$, $\gamma = 1.1$.
		\ENSURE  \{ \(\bZ^{v}, \bW^{v}, \bb^v, \bY \) \},  \(v = 1,\dots, m \), 
		\REPEAT
		\STATE Updating each $\bW^{v}(t+1)$ according to eq.(\ref{solve_w});
		
		\STATE Updating each $\bb^{v}(t+1)$ according to eq.(\ref{solve_b});
		
		\STATE Updating $\bY(t+1)$ according to eq.(\ref{solve_y});
		
		\STATE Updating each $\bZ^{v}(t+1)$ according to eq.(\ref{solve_z});
		
		\STATE t = t + 1.
		\UNTIL {convergence} (e.g., when $||\bY(t+1) - \bY(t)|| \leq \epsilon$ or the maximum iteration T is reached ).
%		
%		\STATE Applying spectral clustering on $\bZ^{*}$ to obtain the final cluster result.
	\end{algorithmic}
	
\end{algorithm}

==> paper/proposed_model/convergence_analysis.tex <==

\subsection{Convergence analysis}

==> paper/proposed_model/optimization.tex <==
\subsection{Optimization}

According to algorithm1, problem (\ref{spl_proposed_model}) can be solved by iteratively solving the following subproblems,
\\
\\
\textbf{P1}, given $\{\{\bZ^v,\bb^v,\bW^v\}_{v=1}^m, \bY\}$, optimizing the sample weights under each view $\{\bp^v\}_{v=1}^m$. The optimum value is determined by the corresponding minimizer function,
\begin{equation}
	\begin{split}
		& (\bp_i^v)^* = \sigma( \ell_i^v, \lambda), \quad v = 1,...,m \ , i = 1 ,...,n \\
		\ell_i^v = & \sqrt{||\bX_i^v - \bX^v \bZ_i^v||^2 
			+ \beta||\bW^v \bX_i^v + \bb^v - \bY_i||^2}.
	\end{split}
\end{equation}
\\
\\
\textbf{P2}, given sample weights $\{\bp^v\}_{v=1}^m$, optimizing the model parameters $\{\{\bZ^v,\bb^v,\bW^v\}_{v=1}^m, \bY\}$. Denoting $\bP^v = diag(\sqrt{\bp^v}), v = 1,...,m$, the minimization problem becomes
\begin{equation}
	\begin{split}
		& \min_{\{\bZ^v,\bb^v,\bW^v\}_{v=1}^m, \bY}  
		H = \frac{1}{2} \sum_{v=1}^{m} \{||(\bX^v - \bX^v \bZ^v)\bP^v||_F^2 \\
		& \quad \quad + \beta ||(\bW^v \bX^v + \bb^v \textbf{1}_n^T - \bY)\bP^v||_F^2 
		+ \rho ||\bZ^v||_\bY\} \\
		& \; s.t. \; \bY\bY^T = \bI, \bZ^v \geq 0, diag(\bZ^v) = \textbf{0},v = 1,...,m. 
	\end{split}
	\label{p2}
\end{equation}
%
This is still a non-convex and non-smooth function which is hard to be optimized. And we develop an iterative algorithm based on the recently developed Proximal Alternating Linearized Minimization method(PALM)\cite{bolte2014proximal,attouch2010proximal}. PALM alternatively optimizes each block of variables while keeping the others fixed, it performs one gradient step on the smooth part followed by a proximal operator on the non-smooth constraints. For ease of representation, we give the definition of the indicator function as
%
\begin{equation}
	\delta_{\bGamma}(\bM) = \left \{
	\begin{split}
		& \ 0, \; \; \; \; \;  \    if \; \bM \in \bGamma \\
		& +\infty, \; otherwise
	\end{split}
	\right.
	\label{indicator_function}
\end{equation}
The proximal map  associated to the indicator function is defined by
\begin{equation}
	prox^{\delta_{\bGamma}}(\bV) = \arg \min_{\bU} \{||\bU - \bV||_F^2, s.t. \bU \in \bGamma \}.
	\label{proximal_map}
\end{equation}
And define 
$\bGamma_1 = \{\bY \in R^{k\times n} : \bY \bY^T =\bI\}$,
$\bGamma_2 = \{\bZ \in R^{n\times n} : \bZ = \bZ^T, diag(\bZ) = 0, \bZ_{ij} \geq 0, i,j=1,...,n\}$.
The whole optimization procedure of (\ref{p2}) is given below.
%
\\ \\
%
\textbf{$\bW$-step} Update each $\bW^v(t+1)$ with fixed $\{\{\bZ^v(t),\bb^v(t),\bW^v(t)\}_{v=1}^m,\bY(t)\}$, $t$ is the iteration number. 
Denote $\bA = [A^1;...;A^m] \in R^{ (mk) \times n}$ with $\bA^v = (\bY - \bb^v \textbf{1}_n^T)\bP^v$, 
$\bB = [B^1;...;B^m] \in R^{d\times n}$ with $\bB^v = \bX^{v} \bP^v$, and 
\begin{equation*}       
	\bW = \left [              
	\begin{array}{ccc}   
		\bW^{1} & \cdots & \textbf{0}\\  
		\vdots & \ddots & \vdots\\  
		\textbf{0} & \cdots & \bW^{m}
	\end{array}
	\right].       
\end{equation*}
Problem(\ref{spl_proposed_model}) equals to
\begin{equation}
	\min_{\bW \in R^{(mk)\times (md)}} \; J = \frac{1}{2} ||\bW \bB - \bA||_F^2 .
\end{equation}
Taking the partial derivatives of $J$ with respect to $\bW$, we obtain that
\begin{equation}
	\triangledown_\bW J = \bW \bB \bB^T - \bA^T \bB^T
\end{equation}
The Lipschitz moduli of $\triangledown_\bW J$ is calculated by $\ell_\bW = ||\bB \bB^T||_F$, and $\bW(t+1)$ is determined by solving the following problem,
\begin{equation}
	\min_{\bU \in R^{(mk)\times (md)}} ||\bU - (\bW(t) - \frac{1}{\gamma \ell_\bW}\triangledown_\bW J(\bW(t)))||_F^2,
\end{equation}
which obtains an analytical solution as
\begin{equation}
	\bW(t+1) = \bW(t) - \frac{1}{\gamma \ell_\bW}\triangledown_\bW J(\bW(t)).
	\label{solve_w}
\end{equation}
%
\\ \\
%b-step
\textbf{$\bb$-step} Update each $\bb^v(t+1)$ with fixed $\{\{\bZ^v(t),\bb^v(t),\bW^v(t)\}_{v=1}^m,\bY(t)\}$. Denote $\bF^v = (\bY - \bW^v \bX^v) \bP^v$, problem (\ref{p2}) is equivalent to
\begin{equation}
	\min_{\bb^1,...,\bb^m} J = \frac{1}{2}||\bb^v \textbf{1}_n^T \bP^v - \bF^v||_F^2.
\end{equation}
Taking its partial derivatives with respect to $\bb^v$, we get
\(\triangledown_{\bb^v} J = (\bb^v \textbf{1}_n^T \bP^v - \bF^v) \textbf{1}_n \).
The Lipschitz moduli of $\triangledown_{\bb^v} J$ is $\ell_\bb^v = tr(\bP^v)$. 
And the solution of $\bb^v(t+1)$ is 
\begin{equation}
	\bb^v(t+1) = \bb^v(t) - \frac{1}{\gamma \ell_\bb^v} \triangledown_{\bb^v} J(\bb^v(t)).
	\label{solve_b}
\end{equation}
%
\\ \\
\textbf{$\bY$-step} Update $\bY(t+1)$ with other variables fixed. Problem (\ref{p2}) reduces to
\begin{equation}
\begin{split}
	\min_{\bY \in \bGamma_1} J &= \frac{1}{2}\sum_{v=1}^{m} \{\beta ||\bM^v - \bY \bP^v||_F^2
	+ \rho ||\bZ^v||_\bY \}, \\
\end{split}
\end{equation}
where $\bM^v = (\bW^v \bX^v + \bb^v \textbf{1}_n^T)\bP^v, v=1,...,m$. Denote $\bL^v = \bD^v - \bZ^v$, $\bD^v$ is a diagonal matrix with $\bD_{ii}^v = \sum_{j=1}^{n} \bZ_{ij}^v$, let $\bL^* = \sum_{v=1}^{m} \bL^v$.
Taking the derivatives of $J$ with respect to $\bY$, we obtain
\begin{equation}
\begin{split}
	\triangledown_{\bY} J 
	& = \beta \sum_{v=1}^{m} \{\bY (\bP^v)^2 - \bM^v \bP^v\} + \frac{\rho}{2} \bY (\bL^* + (\bL^*)^T) \\
	& = \bY (\beta \sum_{v=1}^{m} (\bP^v)^2 + \frac{\rho}{2} (\bL^* + (\bL^*)^T)) - \beta \sum_{v=1}^{m} \bM^v \bP^v. \\
\end{split}
\end{equation}
The Lipschitz moduli of $\triangledown_\bY J$ is calculated by $\ell_\bY = ||\beta \sum_{v=1}^{m} (\bP^v)^2 + \frac{\rho}{2} (\bL^* + (\bL^*)^T)||_F$, and we can obtain $\bY(t+1)$ via solving the following proximal problem,
\begin{equation}
\begin{split}
	\bY(t+1) & = prox^{\delta_{\bGamma_{1}}} ( \bY(t) - \frac{1}{c_{y}} \triangledown_{\bY} J(\bY(t)) ),
\end{split}
\label{solve_y}
\end{equation}
where $c_y = \gamma \ell_{\bY}, \gamma > 1$. According to the proximal map of the indicator function, denote $\bV = \bY(t) - \frac{1}{c_{y}} \triangledown_{\bY} J(\bY(t))$, eq(\ref{update_y}) is equivalent to 
\begin{equation}
	\bY(t+1) = \arg \min_{\bU} \{||\bU - \bV||_F^2, \ s.t \ \ \bU \bU^T = \bI. \}
	\label{www}
\end{equation}
This problem admits a closed-form solution according to the Theorem 1 in \cite{wang2013multi}. More specifically, by performing singular value decomposition (SVD) on $\bV = \bS \Lambda \bQ^T$, $\bS \in R^{k \times k}$ and $\bQ \in R^{n \times n}$, the solution of (\ref{www}) is given by 
\begin{equation}
	\bY(t+1) = \bS [\bI, \textbf{0}] \bQ^T,
\end{equation}
where $\bI$ is the identity matrix with size $k$, and \textbf{0} $\in R^{k \times (n-k)}$ is a zero matrix.
%
%Z-step
\\ \\
\textbf{$\bZ$-step} Update each $\bZ^v$ while the other variables are fixed.
Denote $\bC \in R^{n \times n}, \bC_{ij} = ||\bY_i - \bY_j||^2$, problem (\ref{p2}) reduces to
\begin{equation}
\begin{split}
	& \min_{\bZ^1,...,\bZ^m}	J = \frac{1}{2} \sum_{v=1}^{m} \{||(\bX^v - \bX^v \bZ^v)\bP^v||_F^2  + \rho tr(\bZ^v \bC)\} \\
	& \; s.t \;\ \bZ^v \in \bGamma_2, v = 1,...,m .
\end{split}
\end{equation}
Taking the partial derivatives of $J$ with respect to $\bZ^v$, we obtain
\begin{equation}
\begin{split}
	\triangledown_{\bZ^v} J = (\bX^v)^T \bX^v \bZ^v (\bP^v)^2 - (\bX^v)^T \bX^v (\bP^v)^2 + \frac{\lambda}{2} \bC\\
\end{split}
\end{equation}
The Lipschitz moduli of $\triangledown_\bZ^v J$ is calculated by $\ell_\bZ^v = ||\bX^v)^T \bX^v||_F * ||(\bP^v)^2||_F$, and we can obtain $\bZ^v(t+1)$ via solving the following proximal problem,
\begin{equation}
	\bZ^v(t+1) = prox^{\delta_{\bGamma_{2}}} ( \bZ^v(t) - \frac{1}{c_{z^v}} \triangledown_{\bZ^v} J(\bZ^v(t)) ),
\label{update_z}
\end{equation}
where $c_{z^v} = \gamma \ell_{\bZ^v}, \gamma > 1$. According to (\ref{proximal_map}), denote $\bV^v = \bZ^v(t) - \frac{1}{c_{z^v}} \triangledown_{\bZ^v} J(\bZ^v(t)) $, eq(\ref{update_z}) is equivalent to 
\begin{equation}
\bZ^v(t+1) = \arg \min_{\bU} \{||\bU - \bV^v||_F^2, \ s.t \ \ \bU \in \bGamma_2. \},
\end{equation}
which has a closed-form solution as
\begin{equation}
	\bZ^v = \left \{
	\begin{split}
	& \max(0, \bV_{ij}^v), \; \; \; \; \;  \    if \; i \neq j\\
	& \ 0, \; \; \; \; \quad \quad \quad \quad \quad otherwise
	\end{split}
\right.
\label{solve_z}
\end{equation}
%
The whole optimization procedure of \textbf{P2} is summarized in Algorithm \ref{alg_for_p2}. 
After obtaining the optimal solution, the final clustering results can be achieved by directly running k-means cluster on the learned $\bY$ or via spectral clustering methods like \cite{shi2000normalized} on $\bZ^v$. 

==> paper/proposed_model/problem_formulation.tex <==
\subsection{Problem Formulation}

Recently developed spectral clustering based subspace clustering methods mainly follow a two-stage strategy. That is, they first learn an affinity matrix based on the data's self-representation and some structure priors, then the spectral clustering algorithm like \cite{shi2000normalized} is applied to the learned affinity matrix for the final clustering results. Methods that based on this strategy have achieved promising results\cite{hu2014smooth,liu2010robust,elhamifar2013sparse,liu2013robust,wang2013provable,cao2015diversity}. However, due to fact that the clustering results and the learned affinity matrix are related to each other, this two-step approach is sub-optimal. Based on this, \cite{Li_2015_CVPR} propose a unified framework which combines the learned affinity matrix and the final clustering results via a subspace structured norm.
Meanwhile, according to the results in \cite{nie2009spectral}, the true cluster assignment matrix can be always embedded into a low dimensional linear mapping of the data. Therefore, the cluster assignment $\bY$ is expect to be close to a linear space spanned by the data $\bX$.
%
Inspired by these advance, we develop a novel multi-view clustering model that formulated as 
\begin{equation}
\begin{split}
	& \min \; \frac{1}{2}\sum_{v=1}^{m}
	\{||\bX^v - \bX^v \bZ^v||_F^2 \\
	& \quad \quad \quad \quad  + \beta ||\bW^v \bX^v + \bb^v \textbf{1}_n - \bY||_F^2 + \rho ||\bZ^v||_\bY\} \\
	& \; s.t. \; \bY\bY^T = \bI, \bZ^v \geq 0, diag(\bZ^v) = \textbf{0},v = 1,...,m. 
\end{split}
\label{ori_proposed_model}
\end{equation}
%
As it is a non-convex function, we apply the proposed SPIR to optimize it in case of getting stuck into bad local minima. Problem (\ref{ori_proposed_model}) is reformulated as
%
\begin{equation}
\begin{split}
		&\min \; \frac{1}{2} 
		\sum_{v=1}^{m} \{ ||(\bX^v - \bX^v \bZ^v)diag(\sqrt{\bp_1^v})||_F^2 \\
		&\quad \quad + \beta ||(\bW^v \bX^v + \bb^v \textbf{1}_n - \bY)diag(\sqrt{\bp_2^v})||_F^2 \\
		&\quad \quad  + \rho ||\bZ^v||_\bY  + \psi(\bp_1^v,\bp_2^v) \} \\
		& \ s.t. \; \bY\bY^T = \bI, \bZ^v \geq 0, diag(\bZ^v) = \textbf{0},v = 1,...,m. 
\end{split}
\label{spl_proposed_model}
\end{equation}
%


==> paper/proposed_model/proposed_model.tex <==

\section{SPIR for Multi-view Clustering}

To demonstrate the effectiveness of the proposed self-paced learning framework, we apply it to the task of multi-view clustering. 

\input{paper/proposed_model/problem_formulation}
\input{paper/proposed_model/optimization}
\input{paper/proposed_model/convergence_analysis}
\input{paper/proposed_model/algorithm}



==> paper/table/existed_spl_regularizer.tex <==

\begin{table}
\footnotesize
\centering
\caption{Recently Proposed Self-paced Regularizers and their Corresponding Minimizer Functions}
\label{existed_spl_regularizer}
\setlength\tabcolsep{2pt}
\begin{tabular}{|l|l|l|}

%
%regularization and minimization function
\hline
	& Self-paced Regularizer $g(.)$	& Minimizer Function $\sigma(.)$ \\


%hard
\hline
Kumar \etal \cite{kumar2010self}
& 	

$-\lambda \sum_{i=1}^{n} v_i,\ \lambda>0$

&
$\left\{ {\begin{array}{*{20}{c}}
	1, &  \ell_i < \lambda \\
	0, &  otherwise
	\end{array}} 
\right.$
\\


%linear
\hline
Lu Jiang \etal \cite{jiang2014easy,jiang2015self}

&
$\frac{1}{2} \lambda \sum_{i=1}^{n} (v_i^2 - 2v_i), \ \lambda > 0 $

&
$\left\{ {\begin{array}{*{20}{c}}
	1 - \frac{1}{\lambda}\ell_i, &  \ell_i < \lambda \\
	0, &  otherwise
	\end{array}} 
\right.$
\\

%logarithmic
\hline
Lu Jiang \etal \cite{jiang2014easy,jiang2015self}

&
$\begin{aligned}
&\sum_{i=1}^{n}( \zeta v_i - \frac{\zeta^{v_i}}{\log \zeta}), \\
&\zeta = 1 - \lambda, 0 < \lambda < 1 
\end{aligned}$

&
$\left\{ {\begin{array}{*{20}{c}}
	\frac{1}{\log \zeta} \log(\ell_i + \zeta), &  \ell_i < \lambda \\
	0, &  otherwise
	\end{array}} 
\right.$
\\


%mixture
\hline
{Lu Jiang \etal \cite{jiang2014easy,jiang2015self} }

&

$\begin{aligned}
&-\zeta \sum_{i=1}^{n}\log(v_i + \frac{1}{\lambda_1}\zeta), \\
&\zeta = \frac{\lambda_1 \lambda_2}{\lambda_1 - \lambda_2}, \lambda_1 > \lambda_2 >0
\end{aligned}
$

&
$\left\{ {\begin{array}{*{20}{c}}
	1, &  \ell_i \leq \lambda_2 \\
	\frac{(\lambda_1 - \ell_i)\zeta}{\ell_i \lambda_1}, & \lambda_2 < \ell_i < \lambda_1 \\
	0, &  \ell_i \geq \lambda_1
	\end{array}} 
\right.$
\\

%diversity
\hline
Lu Jiang \etal \cite{jiang2014self}

&
$-\lambda\sum_{i=1}^{n} v_i - \gamma||\bv||_{2,1}, \ \lambda > 0, \ \gamma > 0$

&
$\left\{ {\begin{array}{*{20}{c}}
	1, &  \ell_i \leq \lambda + \gamma \frac{1}{\sqrt{i} - \sqrt{i-1}} \\
	0, &  otherwise
	\end{array}} 
\right.$
\\


%multi-view clustering
\hline
Chang Xu \etal \cite{xu2015multi}

&
$\begin{aligned}
&\sum_{i=1}^{n} \ln(1 + e^{-\lambda} - v_i)^{(1 + e^{-\lambda} - v_i)} \\
&+ \ln(v_i)^{v_i} - \lambda v_i, \ \lambda > 0
\end{aligned}$

&
$\frac{1 + e^{-\lambda}}{1 + e^{\ell_i - \lambda}}$
\\

%matric factorization
\hline
Qian Zhao \etal \cite{zhao2015self}

&
$\sum_{i=1}^{n} \frac{\lambda \gamma^2}{\lambda v_i + \gamma}, \ \lambda > 0, \ \gamma > 0$

&
$\left\{ {\begin{array}{*{20}{c}}
	1, &  \ell_i \leq (\frac{\lambda \gamma}{\lambda + \gamma})^2 \\
	0, &  \ell_i \geq \lambda^2 \\
	\gamma (\frac{1}{\sqrt{\ell_i}} - \frac{1}{\lambda}), & otherwise 
	\end{array}} 
\right.$
\\


%co-saliency detection
\hline
Zhang \etal \cite{zhang2015self}

&
$\begin{aligned}
&-\lambda \sum_{k=1}^{K} \sum_{i=1}^{n_k} v_i^k -\gamma \sum_{k=1}^{K} \sqrt{\sum_{i=1}^{n_k} v_i^k},\\
&\lambda > 0, \ \gamma > 0
\end{aligned}$

&
$\left\{ {\begin{array}{*{20}{c}}
	1, &  \ell_i^k < \lambda + \frac{\gamma}{2\sqrt{i}} \\
	\frac{((\frac{\gamma}{2(\ell_i^k-\lambda)})^2 - (i-1)}{m}, &  otherwise
	\end{array}} 
\right.$
\\
\hline
\end{tabular}
%
\end{table}


==> paper/table/implicit_spl_regularizer_1.tex <==

\begin{table*}
\footnotesize
\centering
\caption{   Loss Function $\phi(.)$ and the Corresponding Minimizer Function $\sigma(.)$, $\lambda$ is a hyper-parameter. }
\label{implicit_spl_regularizer}
\setlength\tabcolsep{2pt}
\begin{tabular}{|c|c|c|c|c|}

%
%regularization and minimization function
\hline
	& Huber	& Cauchy & L1-L2 & Welsch\\

\hline
Loss function $\phi(\lambda,t)$  
& 	
$\left\{ {\begin{array}{*{20}{c}}
	{t,}&{t \leq \lambda }\\
	{\lambda \sqrt{t} - \frac{\lambda^2}{2},}&{t > \lambda}
	\end{array}} 
\right.$

&
$\log(1+t/\lambda^2)$ 

&
$\sqrt{\lambda + t} - 1$ 

&
$1 -\exp(-\frac{t}{\lambda^2})$\\

\hline
Minimizer function $\sigma(\lambda,t)$ 

&
$\left\{ {\begin{array}{*{20}{c}}
	{1}&{|t| \leq \lambda }\\
	{\lambda/|t|,}&{|t| > \lambda}
	\end{array}} 
\right.$

&
$1 / (1+(t/\lambda)^2)$ 

&
$\frac{1}{\sqrt{\lambda + t^2}}$ 

&
$\exp(-\frac{t^2}{\lambda^2})$ \\

\hline
\end{tabular}
%
\end{table*}

==> paper/table/table_mvc_small.tex <==
\begin{table}[!tb]
	\footnotesize
	\centering
	\caption{
	\small{Clustering performance on the Handwritten Digit dataset. The best results are highlighted in bold.}
	}
	\label{result_mvc}
%	\setlength\tabcolsep{5pt}
%	\setlength{\abovecaptionskip}{0.cm}
%	\setlength{\belowcaptionskip}{-10.cm}
%	\begin{tabular}{|l|c|c|c|}
	\begin{tabular}{c| c c c}

		\hline
		Method & ACC & NMI & AR \\
		\hline
		
		BSV & 0.734(0.062) &	 0.730(0.030) &	 0.634(0.055)  \\
		\hline			
		Con-MC & 0.775(0.078) &	 0.773(0.037) &	 0.690(0.066) \\
		\hline
		
		\tabincell{c}{SPL-hard} & 0.821(0.059) &	 0.758(0.029) &	 0.709(0.050) \\
		\hline
		
%		\tabincell{c}{SPL-linear} & 0.838(0.069) &	 0.805(0.034) &	 0.749(0.062) \\
%		\hline
		
		\tabincell{c}{SPL-mixture} & 0.845(0.068) &	 0.812(0.030) &	 0.763(0.057) \\
		\hline
		
		{\tabincell{c}{MSPL}} & 0.840(0.070) &	 0.806(0.035) &	 0.751(0.064) \\
		\hline
		
		SPL-IR-huber & 0.843(0.070)	& 0.810(0.035)	& 0.756(0.064)	\\
		\hline
		
		
		SPL-IR-L1-L2 & 0.835(0.068)	& 0.801(0.034)	& 0.743(0.061)	\\
		\hline
		
		SPL-IR-cauchy & {0.845}(0.071) & {0.814}(0.035) &	 {0.762}(0.064) 	 \\
		\hline
		
		SPL-IR-welsch & \textbf{0.862(0.071)}	& \textbf{0.833(0.035)}	& \textbf{0.790(0.064)}	\\
		
		\hline
%		- & - & - & - & SPL-IR-cauchy & 0 & 0 & 0 \\
%		\hline
	\end{tabular}
\end{table}
